Is user feedback always informative? Retrieval Latent Defending for Semi-Supervised Domain Adaptation without Source Data

This paper aims to adapt the source model to the target environment, leveraging small user feedback (i.e., labeled target data) readily available in real-world applications. We find that existing semi-supervised domain adaptation (SemiSDA) methods often suffer from poorly improved adaptation performance when directly utilizing such feedback data, as shown in Figure 1. We analyze this phenomenon via a novel concept called Negatively Biased Feedback (NBF), which stems from the observation that user feedback is more likely for data points where the model produces incorrect predictions. To leverage this feedback while avoiding the issue, we propose a scalable adapting approach, Retrieval Latent Defending. This approach helps existing SemiSDA methods to adapt the model with a balanced supervised signal by utilizing latent defending samples throughout the adaptation process. We demonstrate the problem caused by NBF and the efficacy of our approach across various benchmarks, including image classification, semantic segmentation, and a real-world medical imaging application. Our extensive experiments reveal that integrating our approach with multiple state-of-the-art SemiSDA methods leads to significant performance improvements.

==> fig/cab_tsne.tex <==
\begin{figure}[t]\centering
\vspace{-0.5em}
\includegraphics[width=0.99\linewidth]{img/CaB_tsne.pdf}
\vspace{-0.5em}
\caption{\textbf{Effect of class-aware balancing on DomainNet.} 
We analyze our method using t-SNE visualization, in which we only adapt the classifier to the real domain while freezing the backbone of the pretrained model on the painting domain (\ie, linear-probing). Regardless of the biased label distribution, our method helps the model to predict samples within class clusters more correctly.}
\label{fig:cabtsne}
\vspace{-0.5em}
\end{figure}

==> fig/global_shape.tex <==
\begin{figure}[t]\centering
% \vspace{-.5em}
\includegraphics[width=0.95\linewidth]{img/global_shape}
\vspace{-1.2em}
\caption{We illustrate model adapting without (left) and with (right) our approach. When labeled samples are biasedly positioned,
our balancing sample $x_{CaB}$ helps the model to be adapted with balanced class discriminability (\ie, decision boundary).}
\label{fig:globalshape}
\vspace{-1.5em}
\end{figure}

% our approach helps state-of-the-art methods to achieve better performance by preventing the mini-batch from becoming overly dependent on the biased feedback.
